Spectral Learning for Supervised Topic Models

Supervised topic models simultaneously model the latent topic structure of large collections of documents and a response variable associated with each document. Existing inference methods are based on variational approximation or Monte Carlo sampling, which often suffers from the local minimum defect. Spectral methods have been applied to learn unsupervised topic models, such as latent Dirichlet allocation (LDA), with provable guarantees. This paper investigates the possibility of applying spectral methods to recover the parameters of supervised LDA (sLDA). We first present a two-stage spectral method, which recovers the parameters of LDA followed by a power update method to recover the regression model parameters. Then, we further present a single-phase spectral algorithm to jointly recover the topic distribution matrix as well as the regression weights. Our spectral algorithms are provably correct and computationally efficient. We prove a sample complexity bound for each algorithm and subsequently derive a sufficient condition for the identifiability of sLDA. Thorough experiments on synthetic and real-world datasets verify the theory and demonstrate the practical effectiveness of the spectral algorithms. In fact, our results on a large-scale review rating dataset demonstrate that our single-phase spectral algorithm alone gets comparable or even better performance than state-of-the-art methods, while previous work on spectral methods has rarely reported such promising performance.

==> Makefile <==
TARGET=spectral-slda
TEX=xelatex -shell-escape
BIBTEX=bibtex 
READER=evince

all: view

rebuild  output/$(TARGET).pdf: *.tex *.bib output
	cp -r fig output/ && cp -r images output/  && cd output && rm -f *.tex *.bib && ln -s ../*.tex ../*.bib .
	cd output && $(TEX) $(TARGET).tex && $(BIBTEX)$ $(TARGET).aux && \
		$(TEX) $(TARGET).tex  && $(TEX) $(TARGET).tex
	make

output: 
	mkdir output
	cd output && rm -f data src && ln -s ../data ../src .

view: output/$(TARGET).pdf
#	$(READER) output/$(TARGET).pdf &

clean:
	rm -rf output

.PHONY: all view clean rebuild dist


==> untitled folder/Makefile <==
TARGET=spectral-slda
TEX=xelatex -shell-escape
BIBTEX=bibtex 
READER=evince

all: view

rebuild  output/$(TARGET).pdf: *.tex *.bib output
	cp -r fig output/ && cp -r images output/  && cd output && rm -f *.tex *.bib && ln -s ../*.tex ../*.bib .
	cd output && $(TEX) $(TARGET).tex && $(BIBTEX)$ $(TARGET).aux && \
		$(TEX) $(TARGET).tex  && $(TEX) $(TARGET).tex
	make

output: 
	mkdir output
	cd output && rm -f data src && ln -s ../data ../src .

view: output/$(TARGET).pdf
#	$(READER) output/$(TARGET).pdf &

clean:
	rm -rf output

.PHONY: all view clean rebuild dist


==> untitled folder/supplementary1.tex <==
\section{Proof to Theorem 1}
In this section, we prove the sample complexity bound given in Theorem 1. The proof consists of three main parts.
In Appendix A.1, we prove perturbation lemmas that bound the estimation error of the whitened tensors
$M_2(W,W), M_y(W,W)$ and $M_3(W,W,W)$ in terms of the estimation error of the tensors themselves.
In Appendix A.2, we cite results on the accuracy of SVD and robust tensor power method when performed on estimated tensors,
and prove the effectiveness of the power update method used in recovering the linear regression model $\vct\eta$.
Finally, we give tail bounds for the estimation error of $M_2,M_y$ and $M_3$ in Appendix A.3
and complete the proof in Appendix A.4.
We also make some remarks on the indirect quantities (e.g. $\sigma_k(\widetilde O)$) used in Theorem 1
and simplified bounds for some special cases in Appendix A.4.

All norms in the following analysis, if not explicitly specified, are 2 norms in the vector and matrix cases and the operator norm in the high-order tensor case.

\subsection{Perturbation lemmas}

We first define the canonical topic distribution vectors $\widetilde{\vct\mu}$ and estimation error of observable tensors,
which simplify the notations that arise in subsequent analysis.

\begin{deff}[canonical topic distribution]
Define the canonical version of topic distribution vector $\vct\mu_i$, $\widetilde{\vct\mu}_i$, as follows:
\begin{equation}
\widetilde{\vct\mu}_i \triangleq \sqrt{\frac{\alpha_i}{\alpha_0(\alpha_0+1)}}\vct\mu_i.
\label{def_can_mu}
\end{equation}

We also define $O,\widetilde O\in\mathbb R^{n\times k}$ by $O = [\vct\mu_1,\cdots,\vct\mu_k]$ and $\widetilde{O} = [\widetilde{\vct\mu_1},\cdots,\widetilde{\vct\mu_k}]$.
\end{deff}

\begin{deff}[estimation error]
Assume
\begin{eqnarray}
\|M_2-\widehat M_2\| &\leq& E_P,\\
\|M_y-\widehat M_y\| &\leq& E_y,\\
\|M_3-\widehat M_3\| &\leq& E_T.
\end{eqnarray}
for some real values $E_P,E_y$ and $E_T$, which we will set later.
\end{deff}

The following lemma analyzes the whitening matrix $W$ of $M_2$.
Many conclusions are directly from \cite{a:twosvd}.

\begin{lem}[Lemma C.1, \cite{speclda}]
Let $W, \widehat W\in\mathbb R^{n\times k}$ be the whitening matrices such that $M_2(W,W) = \widehat M_2(\widehat W,\widehat W) = I_k$. Let $A = W^\top\widetilde O$ and $\widehat A = \widehat W^\top\widetilde O$. Suppose $E_P \leq \sigma_k(M_2)/2$. We have
\begin{eqnarray}
\|W\| &=& \frac{1}{\sigma_k(\widetilde O)},\\
\|\widehat W\| &\leq& \frac{2}{\sigma_k(\widetilde O)},\label{eq6_pert}\\
\|W-\widehat W\| &\leq& \frac{4E_P}{\sigma_k(\widetilde O)^3},\label{eq_wwhat}\\
\|W^+\| &\leq& 3\sigma_1(\widetilde O),\\
\|\widehat W^+\| &\leq& 2\sigma_1(\widetilde O),\\
\|W^+ - \widehat W^+\| &\leq& \frac{6\sigma_1(\widetilde O)}{\sigma_k(\widetilde O)^2}E_P,\\
\|A\| &=& 1,\\
\|\widehat A\| &\leq & 2,\\
\|A - \widehat A\| &\leq& \frac{4E_P}{\sigma_k(\widetilde O)^2},\\
\|AA^\top - \widehat A\widehat A^\top\| &\leq& \frac{12E_P}{\sigma_k(\widetilde O)^2}.\label{eq4_pert}
\end{eqnarray}
\label{lem_whiten}
\end{lem}

\begin{proof}
Proof to Eq. (\ref{eq_wwhat}):
Let $\widehat W^\top\widehat M_2\widehat W = I$ and $\widehat W^\top M_2\widehat W = BDB^\top$, where $B$ is orthogonal and $D$ is a positive definite diagonal matrix.
We then see that $W = \widehat WBD^{-1/2}B^\top$ satisfies the condition $W M_2 W^\top = I$.
Subsequently, $\widehat W = WBD^{1/2}B^\top$.
We then can bound $\|W-\widehat W\|$ as follows
$$ \|W-\widehat W\| \leq \|W\|\cdot \|I-D^{1/2}\| \leq \|W\|\cdot \|I-D\| \leq \frac{4E_P}{\sigma_k(\widetilde O)^3},$$
where the inequality $\|I-D\|\leq \frac{4E_P}{\sigma_k(\widetilde O)^2}$ was proved in \cite{speclda}.

Proof to Eq. (\ref{eq4_pert}):
$\|AA^\top-\widehat A\widehat A^\top\| \leq \|AA^\top-A\widehat A^\top\| + \|A\widehat A^\top - \widehat A\widehat A^\top\|
\leq \|A-\widehat A\|\cdot (\|A\|+\|\widehat A\|) \leq \frac{12E_P}{\sigma_k(\widetilde O)^2}$.

All the other inequalities come from Lemma C.1, \cite{speclda}.
\end{proof}

We are now able to provide perturbation bounds for estimation error of whitened moments.

\begin{deff}[estimation error of whitened moments]
Define
\begin{eqnarray}
\varepsilon_{p,w} &\triangleq& \|M_2(W, W) - \widehat M_2(\widehat W,\widehat W)\|,\\
\varepsilon_{y,w} &\triangleq& \|M_y(W, W) - \widehat M_y(\widehat W,\widehat W)\|,\\
\varepsilon_{t,w} &\triangleq& \|M_3(W,W,W) - \widehat M_3(\widehat W,\widehat W,\widehat W)\|.
\end{eqnarray}
\label{def_epsilon}
\end{deff}
\begin{lem}[Perturbation lemma of whitened moments]
Suppose $E_P\leq \sigma_k(M_2)/2$. We have
\begin{eqnarray}
\varepsilon_{p,w} &\leq& \frac{16E_P}{\sigma_k(\widetilde O)^2},\\
\varepsilon_{y,w} &\leq& \frac{24\|\vct\eta\|E_P}{(\alpha_0+2)\sigma_k(\widetilde O)^2} + \frac{4E_y}{\sigma_k(\widetilde O)^2},\\
\varepsilon_{t,w} &\leq& \frac{54E_P}{(\alpha_0+1)(\alpha_0+2)\sigma_k(\widetilde O)^5} + \frac{8E_T}{\sigma_k(\widetilde O)^3}.
\end{eqnarray}
\end{lem}

\begin{proof}
Using the idea in the proof of Lemma C.2 in \cite{speclda}, we can split $\varepsilon_{p,w}$ as
\begin{equation*}
\begin{aligned}
	\varepsilon_{p,w}
	=& \|M_2(W,W) - M_2(\widehat W,\widehat W) + M_2(\widehat W,\widehat W) - \widehat M_2(\widehat W,\widehat W)\|\\
\leq& \|M_2(W,W) - M_2(\widehat W,\widehat W)\| + \|M_2(\widehat W,\widehat W) - \widehat M_2(\widehat W,\widehat W)\|.
\end{aligned}
\end{equation*}

We can the bound the two terms seperately, as follows.

%\junx{How to split? Sum? please make it clear.}

For the first term, we have
\setlength\arraycolsep{1pt}\begin{eqnarray*}
\|M_2(W,W) - M_2(\widehat W,\widehat W)\|
&=& \|W^\top M_2 W-\widehat W^\top\widehat M_2\widehat W\|\\
&=& \|AA^\top - \widehat A\widehat A^\top\|\\
&\leq& \frac{12E_P}{\sigma_k(\widetilde O)^2}.
\end{eqnarray*}
where the last inequality comes from Eq. (\ref{eq4_pert}).

For the second term, we have
$$\|M_2(\widehat W,\widehat W)-\widehat M_2(\widehat W,\widehat W)\| \leq \|\widehat W\|^2\cdot \|M_2-\widehat M_2\| \leq \frac{4E_P}{\sigma_k(\widetilde O)^2},$$
where the last inequality comes from Eq. (\ref{eq6_pert}).
%\junx{where the last inequality comes from Eq. (6)?}

Similarly, $\varepsilon_{y,w}$ can be splitted as $\|M_y(W,W)-M_y(\widehat W,\widehat W)\|$ and $\|M_y(\widehat W,\widehat W)-\widehat M_y(\widehat W,\widehat W)\|$, which can be bounded separately. For the first term, we have
\begin{equation*}
\begin{aligned}
	\|M_y(W,W) - M_y(\widehat W,\widehat W)\|
	=& \|W^\top M_y W - \widehat W^\top M_y\widehat W\|\\
=& \frac{2}{\alpha_0+2}\|A\diag(\vct\eta)A^\top - \widehat A\diag(\vct\eta)\widehat A^\top\|\\
\leq& \frac{2\|\vct\eta\|}{\alpha_0+2}\cdot \|AA^\top - \widehat A\widehat A^\top\|\\
\leq& \frac{24\|\vct\eta\|}{(\alpha_0+2)\sigma_k(\widetilde O)^2}\cdot E_P.
\end{aligned}
\end{equation*}

For the second term, we have
$$\|M_y(\widehat W,\widehat W)-\widehat M_y(\widehat W,\widehat W)\| \leq \|\widehat W\|^2\cdot\|M_y-\widehat M_y\| \leq \frac{4E_y}{\sigma_k(\widetilde O)^2}.$$

Finally, we bound $\varepsilon_{t,w}$ as below, following the work \cite{specregression}.

\begin{eqnarray*}
\varepsilon_{t,w} &=& \|M_3(W,W,W) - \widehat M_3(\widehat W,\widehat W,\widehat W)\|\\
&\leq& \|M_3\|\cdot \|W-\widehat W\|\cdot (\|W\|^2 + \|W\|\cdot \|\widehat W\|
 + \|\widehat W\|^2) + \|\widehat W\|^3\cdot \|M_3-\widehat M_3\|\\
&\leq& \frac{54E_P}{(\alpha_0+1)(\alpha_0+2)\sigma_k(\widetilde O)^5} + \frac{8E_T}{\sigma_k(\widetilde O)^3},
\end{eqnarray*}
where we have used the fact that $$\|M_3\| \leq \sum_{i=1}^k{\frac{2\alpha_i}{\alpha_0(\alpha_0+1)(\alpha_0+2)}} = \frac{2}{(\alpha_0+1)(\alpha_0+2)}.$$

\end{proof}

\subsection{SVD accuracy}

The key idea for spectral recovery of LDA topic modeling is the \emph{simultaneous diagonalization} trick,
which asserts that we can recover LDA model parameters by performing orthogonal tensor decomposition
on a pair of simultaneously whitened moments, for example, $(M_2, M_3)$ and $(M_2, M_y)$.
The following proposition details this insight, as we derive orthogonal tensor decompositions for the whitened tensor product
$M_y(W,W)$ and $M_3(W,W,W)$.

\begin{prop}
Define $\vct v_i\triangleq W^\top \widetilde{\vct\mu}_i = \sqrt{\frac{\alpha_i}{\alpha_0(\alpha_0+1)}}W^\top\vct\mu_i$. Then
\begin{enumerate}
\item $\{\vct v_i\}_{i=1}^k$ is an orthonormal basis.
\item $M_y$ has a pair of singular value and singular vector $(\sigma_i^y, \vct v_i)$ with $\sigma_i^y = \frac{2}{\alpha_0+2}\eta_j$ for some $j \in[k]$.
\item $M_3$ has a pair of robust eigenvalue and eigenvector \cite{a:tensordecomp} $(\lambda_i, \vct v_i)$ with $\lambda_i = \frac{2}{\alpha_0+2}\sqrt{\frac{\alpha_0(\alpha_0+1)}{\alpha_{j'}}}$ for some $j'\in[k]$.
\end{enumerate}
\end{prop}

\begin{proof}
The orthonormality of $\{\vct v_i\}_{i=1}^k$ follows from the fact that $W^\top M_2W = \sum_{i=1}^k{\vct v_i\vct v_i^\top} = I_k$.
Subsequently, we have
\setlength\arraycolsep{1pt}\begin{eqnarray*}
M_y(W, W) &=& \frac{2}{\alpha_0+2}\sum_{i=1}^k{\eta_i \vct v_i\vct v_i^\top},\\
M_3(W,W,W) &=& \frac{2}{\alpha_0+2}\sum_{i=1}^k{\sqrt{\frac{\alpha_0(\alpha_0+1)}{\alpha_i}}\vct v_i\otimes\vct v_i\otimes\vct v_i}.
\end{eqnarray*}
\end{proof}

The following lemmas (Lemma \ref{lem_eta} and Lemma \ref{lem_mu})
give upper bounds on the estimation error of $\vct\eta$ and $\vct\mu$
in terms of $|\widehat\lambda_i-\lambda_i|$, $|\widehat{\vct v}_i-\vct v_i|$
and the estimation errors of whitened moments defined in Definition \ref{def_epsilon}.

\begin{lem}[$\eta_i$ estimation error bound]
Define $\widehat\eta_i \triangleq \frac{\alpha_0+2}{2}\widehat{\vct v}_i^\top\widehat M_y(\widehat W,\widehat W)\widehat{\vct v}_i$,
where $\widehat{\vct v}_i$ is some estimation of $\vct v_i$.
We then have
\begin{equation}
|\eta_i - \widehat\eta_i| \leq 2\|\vct\eta\|\|\widehat{\vct v}_i-\vct v_i\| + \frac{\alpha_0+2}{2}(1+2\|\widehat{\vct v}_i-\vct v_i\|)\cdot\varepsilon_{y,w}.
\end{equation}
\label{lem_eta}
\end{lem}

\begin{proof}
First, note that $\vct v_i^\top M_y(W,W)\vct v_i = \frac{2}{\alpha_0+2}\eta_i$ because $\{\vct v_i\}_{i=1}^k$ are orthonormal.
Subsequently, we have
\begin{equation*}
\begin{aligned}
	\frac{2}{\alpha_0+2}|\eta_i - \widehat\eta_i|
	=& \Big|\widehat{\vct v}_i^\top\widehat M_y(\widehat W,\widehat W)\widehat{\vct v}_i - \vct v_i^\top M_y(W,W)\vct v_i\Big| \\
\leq& \Big| (\widehat{\vct v}_i-\vct v_i)^\top \widehat M_y(\widehat W,\widehat W)\widehat{\vct v}_i\Big| + \Big|\vct v_i^\top\left(\widehat M_y(\widehat W,\widehat W)\widehat{\vct v}_i - M_y(W,W)\vct v_i\right)\Big|\\
\leq& \|\widehat{\vct v}_i-\vct v_i\|\|\widehat M_y(\widehat W,\widehat W)\|\|\widehat{\vct v}_i\| + \|\vct v_i\|\|\widehat M_y(\widehat W,\widehat W)\widehat{\vct v}_i - M_y(W,W)\vct v_i\|.\\
\end{aligned}
\end{equation*}

Note that both $\vct v_i$ and $\widehat{\vct v}_i$ are unit vectors. Therefore,
\begin{equation*}
\begin{aligned}
	\frac{2}{\alpha_0+2}|\eta_i-\widehat\eta_i|
\leq& \|\widehat M_y(\widehat W,\widehat W)\|\|\widehat{\vct v}_i-\vct v_i\| + \|\widehat M_y(\widehat W,\widehat W)\widehat{\vct v}_i - M_y(W,W)\vct v_i\|\\
	\leq& \|\widehat M_y(\widehat W,\widehat W)\|\|\widehat{\vct v}_i-\vct v_i\| + \|\widehat M_y(\widehat W,\widehat W)\|\|\widehat{\vct v}_i - \vct v_i\| + \|\widehat M_y(\widehat W,\widehat W)-M_y(W,W)\|\|\vct v_i\|\\
\leq& 2\|\widehat{\vct v}_i-\vct v_i\|\left(\frac{2}{\alpha_0+2}\|\vct\eta\| + \varepsilon_{y,w}\right) + \varepsilon_{y,w}.
\end{aligned}
\end{equation*}

The last inequality is due to the fact that $\|M_y(W,W)\| = \frac{2}{\alpha_0+2}\|\vct\eta\|$.

\end{proof}

\begin{lem}[$\vct\mu_i$ estimation error bound]
Define $\widehat{\vct\mu}_i \triangleq \frac{\alpha_0+2}{2}\widehat\lambda_i(\widehat W^+)^\top\widehat{\vct v}_i$,
where $\widehat\lambda_i, \widehat{\vct v}_i$ are some estimates of singular value pairs $(\lambda_i, \vct v_i)$ of $M_3(W,W,W)$.
We then have
\begin{equation}
\begin{aligned}
	\|\widehat{\vct\mu}_i - \vct\mu_i\| \leq& \frac{3(\alpha_0+2)}{2}\sigma_1(\widetilde O)|\widehat\lambda_i-\lambda_i|
											+ 3\alpha_{\max}\sigma_1(\widetilde O)\|\widehat{\vct v}_i-\vct v_i\|
		+ \frac{6\alpha_{\max}\sigma_1(\widetilde O)E_P}{\sigma_k(\widetilde O)^2}.
\end{aligned}
\end{equation}
\label{lem_mu}
\end{lem}

\begin{proof}
First note that $\vct\mu_i = \frac{\alpha_0+2}{2}\lambda_i (W^+)^\top\vct v_i$. Subsequently,
\begin{equation*}
\begin{aligned}
	\frac{2}{\alpha_0+2}\|\vct\mu_i - \widehat{\vct\mu}_i\|
=& \|\widehat\lambda_i(\widehat W^+)^\top\widehat{\vct v}_i - \lambda_i(W^+)^\top\vct v_i\|\\
\leq& \|\widehat\lambda_i\widehat W^+ - \lambda_i W^+\|\|\widehat{\vct v}_i\| + \|\lambda_i W^+\|\|\widehat{\vct v}_i-\vct v_i\|\\
\leq& |\widehat\lambda_i-\lambda_i|\|\widehat W^+\| + |\lambda_i|\|\widehat W^+ - W^+\| + |\lambda_i|\|W^+\|\|\widehat{\vct v}_i-\vct v_i\|\\
\leq& 3\sigma_1(\widetilde O)|\widehat\lambda_i-\lambda_i| + \frac{2\alpha_{\max}}{\alpha_0+2}\cdot \frac{6\sigma_1(\widetilde O) E_P}{\sigma_k(\widetilde O)^2}
	+ \frac{2\alpha_{\max}}{\alpha_0+2}\cdot 3\sigma_1(\widetilde O)\cdot \|\widehat{\vct v_i} - \vct v_i\|.
\end{aligned}
\end{equation*}
\end{proof}

To bound the error of orthogonal tensor decomposition performed on the estimated tensors $\widehat M_3(\widehat W,\widehat W,\widehat W)$,
we cite Theorem 5.1 \cite{a:tensordecomp}, a sample complexity analysis on the robust tensor power method we used
for recovering $\widehat\lambda_i$ and $\widehat{\vct v}_i$.

\begin{lem}[Theorem 5.1, \cite{a:tensordecomp}]
Let $\lambda_{\max} = \frac{2}{\alpha_0+2}\sqrt{\frac{\alpha_0(\alpha_0+1)}{\alpha_{\min}}}$,
$\lambda_{\min} = \frac{2}{\alpha_0+2}\sqrt{\frac{\alpha_0(\alpha_0+1)}{\alpha_{\max}}}$,
where $\alpha_{\min} = \min{\alpha_i}$ and $\alpha_{\max} = \max{\alpha_i}$.
Then there exist universal constants $C_1, C_2 > 0$ such that the following holds:
Fix $\delta'\in(0,1)$.
Suppose $\varepsilon_{t,w}\leq \varepsilon$ and
\begin{eqnarray}
\varepsilon_{t, w} &\leq& C_1\cdot \frac{\lambda_{\min}}{k},\label{eq1_tensorpower}
\end{eqnarray}
Suppose $\{(\widehat\lambda_i, \widehat{\vct v}_i)\}_{i=1}^k$ are eigenvalue and eigenvector pairs
returned by running Algorithm 1 in \cite{a:tensordecomp} with input $\widehat M_3(\widehat W,\widehat W,\widehat W)$ for $L = \text{poly}(k)\log(1/\delta')$ and $N \geq C_2\cdot(\log(k) + \log\log(\frac{\lambda_{\max}}{\varepsilon}))$ iterations.
With probability greater than $1-\delta'$, there exists a permutation $\pi':[k]\to[k]$ such that
for all $i$,
$$\|\widehat{\vct v}_i - \vct v_{\pi'(i)}\| \leq 8\varepsilon/\lambda_{\min},\quad |\widehat\lambda_i - \lambda_{\pi'(i)}| \leq 5\varepsilon.$$
%\junx{the boldface $\widehat{\vct v}$ or the normal $\widehat{v}$?}
\label{lem_tensorpower}
\end{lem}

\subsection{Tail Inequalities}

\begin{lem}[Lemma 5, \cite{specregression}]
Let $\vct x_1,\cdots,\vct x_N\in\mathbb R^d$ be i.i.d. samples from some distribution with bounded support (i.e., $\|\vct x\|_2\leq B$ with probability 1 for some constant $B$).
%\junx{The main text uses $M$ to denote the document length. Should change one to use a different notation.}{\color{blue}Fixed}
Then with probability at least $1-\delta$,
$$\left\|\frac{1}{N}\sum_{i=1}^N{\vct x_i} - \mathbb E[\vct x]\right\|_2 \leq \frac{2B}{\sqrt{N}}\left(1+\sqrt{\frac{\log(1/\delta)}{2}}\right).$$
\label{lem_chernoff}
\end{lem}

\begin{cor}
Let $\vct x_1,\cdots,\vct x_N\in\mathbb R^d$ be i.i.d. samples from some distributions with $\Pr[\|\vct x\|_2 \leq B] \geq 1-\delta'$.
Then with probability at least $1-N\delta'-\delta$,
$$\left\|\frac{1}{N}\sum_{i=1}^N{\vct x_i} - \mathbb E[\vct x]\right\|_2 \leq \frac{2B}{\sqrt{N}}\left(1+\sqrt{\frac{\log(1/\delta)}{2}}\right).$$
\label{cor_chernoff}
\end{cor}
\begin{proof}
Use union bound.
\end{proof}

\begin{lem}[concentration of moment norms]
Suppose we obtain $N$ i.i.d. samples (i.e., documents with at least three words each and their regression variables in sLDA models).
%Define $R(\delta) \triangleq \|\vct\eta\|+ \Phi^{-1}(\delta)$,
Define $R(\delta) \triangleq \|\vct\eta\| -  \sigma\Phi^{-1}(\delta)$,
where $\Phi^{-1}(\cdot)$ is the inverse function of the CDF of a standard Gaussian distribution.
Let $\mathbb E[\cdot]$ denote the mean of the true underlying distribution
and $\widehat{\mathbb E}[\cdot]$ denote the empirical mean.
Then
\iffalse
\begin{enumerate}
\item $\Pr\left[\|\mathbb E[\vct x_1] - \widehat{\mathbb E}[\vct x_1]\|_F < \frac{2+\sqrt{2\log(1/\delta)}}{\sqrt{N}}\right] \geq 1-\delta$.
\item $\Pr\left[\|\mathbb E[\vct x_1\otimes\vct x_2] - \widehat{\mathbb E}[\vct x_1\otimes\vct x_2]\|_F < \frac{2+\sqrt{2\log(1/\delta)}}{\sqrt{N}}\right] \geq 1-\delta$.
\item $\Pr\left[\|\mathbb E[\vct x_1\otimes\vct x_2\otimes\vct x_3] - \widehat{\mathbb E}[\vct x_1\otimes\vct x_2\otimes\vct x_3]\|_F < \frac{2+\sqrt{2\log(1/\delta)}}{\sqrt{N}}\right] \geq 1-\delta$.
\item $\Pr\left[\|\mathbb E[y] - \widehat{\mathbb E}[y]\| < R(\delta/4\sigma N)\cdot\frac{2+\sqrt{2\log(2/\delta)}}{\sqrt{N}} \right] \geq 1-\delta$.
\item $\Pr\left[\|\mathbb E[y\vct x_1] - \widehat{\mathbb E}[y\vct x_1]\|_F < R(\delta/4\sigma N)\cdot\frac{2+\sqrt{2\log(2/\delta)}}{\sqrt{N}}\right] \geq 1-\delta$.
\item $\Pr\left[\|\mathbb E[y\vct x_1\otimes\vct x_2] - \widehat{\mathbb E}[y\vct x_1\otimes\vct x_2]\|_F < R(\delta/4\sigma N)\cdot\frac{2+\sqrt{2\log(2/\delta)}}{\sqrt{N}}\right] \geq 1 - \delta$.
\end{enumerate}
\fi

\begin{equation}
\begin{aligned}
	& \Pr \left [\|\mathbb E[\vct x_1] - \widehat{\mathbb E}[\vct x_1]\|_F < \frac{2+\sqrt{2\log(1/\delta)}}{\sqrt{N}} \right ] \geq 1-\delta,\\
	&\Pr \left [\|\mathbb E[\vct x_1\otimes\vct x_2] - \widehat{\mathbb E}[\vct x_1\otimes\vct x_2]\|_F < \frac{2+\sqrt{2\log(1/\delta)}}{\sqrt{N}} \right ] \geq 1-\delta,\\
	&\Pr \left [\|\mathbb E[\vct x_1\otimes\vct x_2\otimes\vct x_3] - \widehat{\mathbb E}[\vct x_1\otimes\vct x_2\otimes\vct x_3]\|_F< \frac{2+\sqrt{2\log(1/\delta)}}{\sqrt{N}} \right ] \geq 1-\delta,\\
&\Pr \left [\|\mathbb E[y] - \widehat{\mathbb E}[y]\| < R(\delta/4 N)\cdot\frac{2+\sqrt{2\log(2/\delta)}}{\sqrt{N}} \right ] \geq 1-\delta,\\
&\Pr \left [\|\mathbb E[y\vct x_1] - \widehat{\mathbb E}[y\vct x_1]\|_F < R(\delta/4 N)\cdot\frac{2+\sqrt{2\log(2/\delta)}}{\sqrt{N}} \right ] \geq 1-\delta,\\
&\Pr \left [\|\mathbb E[y\vct x_1\otimes\vct x_2] - \widehat{\mathbb E}[y\vct x_1\otimes\vct x_2]\|_F  < R(\delta/4 N)\cdot\frac{2+\sqrt{2\log(2/\delta)}}{\sqrt{N}} \right ] \geq 1 - \delta.
\end{aligned}
\end{equation}
\label{lem_tail_ineq}
\end{lem}

\begin{proof}
Use Lemma \ref{lem_chernoff} and Corrolary \ref{cor_chernoff} for concentration bounds involving the regression variable $y$.
\end{proof}

\begin{cor}
With probability $1-\delta$ the following holds:
\begin{enumerate}
\item $E_P = \|M_2-\widehat M_2\| \leq 3\cdot \frac{2+\sqrt{2\log(6/\delta)}}{\sqrt{N}}$.
\item $E_y = \|M_y-\widehat M_y\| \leq 10R(\delta/60 N)\cdot \frac{2+\sqrt{2\log(15/\delta)}}{\sqrt{N}}$.
\item $E_T = \|M_3-\widehat M_3\| \leq 10\cdot \frac{2+\sqrt{2\log(9/\delta)}}{\sqrt{N}}$.
\end{enumerate}
\label{cor_ep}
\end{cor}

\begin{proof}
Corrolary \ref{cor_ep} can be proved by expanding the terms by definition and then using tail inequality in Lemma \ref{lem_tail_ineq} and union bound.
Also note that $\|\cdot\| \leq \|\cdot\|_F$ for all matrices.
\end{proof}

\subsection{Completing the proof}

We are now ready to give a complete proof to Theorem \ref{thm_main}.%\jun{should be Theorem 1, right?}

\iffalse
\jun{the following restatement of the theorem is not necessary. Refer to the theorem in the main text. If restating, make them consistent.}
\begin{thm}[Sample complexity bound]
Let $\sigma_1(\widetilde O)$ and $\sigma_k(\widetilde O)$ be the largest and the smallest singular values of the canonical topic distribution matrix $\widetilde O$.
Define $\lambda_{\min} \triangleq \frac{2}{\alpha_0+2}\sqrt{\frac{\alpha_0(\alpha_0+1)}{\alpha_{\max}}}$
and $\lambda_{\max} \triangleq \frac{2}{\alpha_0+2}\sqrt{\frac{\alpha_0(\alpha_0+1)}{\alpha_{\min}}}$，
where $\alpha_{\max}$ and $\alpha_{\min}$ are the largest and the smallest entries in $\vct\alpha$.
Suppose $\widehat{\vct\mu}$, $\widehat{\vct\alpha}$ and $\widehat{\vct\eta}$ are the outputs of Algorithm 1,
%and $L = \poly(k)$ for some low-order polynomial function on $k$.
and $L$ is at least a linear function in $k$.
Fix $\delta\in(0,1)$.
For any small error-tolerance parameter $\varepsilon > 0$,
if Algorithm 1 is run with parameter $T = \Omega(\log(k) + \log\log(\lambda_{\max}/\varepsilon))$
on $N$ i.i.d. sampled documents with
$N\geq \max(n_1, n_2, n_3)$, where
\setlength\arraycolsep{1pt} \begin{eqnarray}
n_1 &=& C_1\cdot \left(1+\sqrt{\log(6/\delta)}\right)^2\cdot \frac{\alpha_0^2(\alpha_0+1)^2}{\alpha_{\min}}, \label{eq_n1} \\
n_2 &=& C_2\cdot \frac{(1+\sqrt{\log(15/\delta)})^2}{\varepsilon^2\sigma_k(\widetilde O)^4}
\\
&\ &\cdot\max\left((\|\vct\eta\| + \Phi^{-1}(\delta/60\sigma))^2, \alpha_{\max}^2\sigma_1(\widetilde O)^2\right),
\label{eq_n2} \\
n_3 &=& C_3\cdot \frac{(1+\sqrt{\log(9/\delta)})^2}{\sigma_k(\widetilde O)^{10}}\cdot\max\left(\frac{1}{\varepsilon^2}, \frac{k^2}{\lambda_{\min}^2}\right),
\label{eq_n3}
\end{eqnarray}
and $C_1, C_2$ and $C_3$ are universal constants,
then with probability at least $1-\delta$, there exists a permutation $\pi:[k]\to [k]$ such that for every topic $i$, the following holds:\\

\begin{enumerate}
\item $|\alpha_i-\widehat{\alpha}_{\pi(i)}| \leq \frac{4\alpha_0(\alpha_0+1)(\lambda_{\max}+5\varepsilon)}{(\alpha_0+2)^2\lambda_{\min}^2(\lambda_{\min}-5\varepsilon)^2}\cdot 5\varepsilon$, if $\lambda_{\min} > 5\varepsilon$;\\

\item $\|\vct\mu_i - \widehat{\vct\mu}_{\pi(i)}\| \leq \left(3\sigma_1(\widetilde O)\left(\frac{8\alpha_{\max}}{\lambda_{\min}} + \frac{5(\alpha_0+2)}{2}\right) + 1\right)\varepsilon$;\\
\item $|\eta_i - \widehat\eta_{\pi(i)}| \leq \left(\frac{\|\vct\eta\|}{\lambda_{\min}} + (\alpha_0+2)\right) \varepsilon$.
\end{enumerate}
\label{thm_main}
\end{thm}
\fi

\begin{proof}{(Proof of Theorem ~\ref{thm_main})}
First, the assumption $E_P\leq\sigma_k(M_2)$ is required for error bounds on $\varepsilon_{p,w}, \varepsilon_{y,w}$ and $\varepsilon_{t,w}$.
Noting Corrolary \ref{cor_ep} and the fact that $\sigma_k(M_2) = \frac{\alpha_{\min}}{\alpha_0(\alpha_0+1)}$, we have
$$N = \Omega\left(\frac{\alpha_0^2(\alpha_0+1)^2(1+\sqrt{\log(6/\delta)})^2}{\alpha_{\min}^2}\right).$$
Note that this lower bound does not depend on $k$, $\varepsilon$ and $\sigma_k(\widetilde O)$.

For Lemma \ref{lem_tensorpower} to hold, we need the assumptions that
$\varepsilon_{t,w} \leq \min(\varepsilon, O(\frac{\lambda_{\min}}{k}))$.
These imply $n_3$,
as we expand $\varepsilon_{t,w}$ according to Definition \ref{def_epsilon}
and note the fact that the first term $\frac{54E_P}{(\alpha_0+1)(\alpha_0+2)\sigma_k(\widetilde O)^5}$ dominates the second one.
The $\alpha_0$ is missing in the third requirment $n_3$ because $\alpha_0+1 \geq 1$, $\alpha_0+2 \geq 2$ and we discard them both.
The $|\alpha_i-\widehat{\alpha}_{\pi(i)}|$ bound follows immediately by Lemma \ref{lem_tensorpower}
and the recovery rule $\widehat{\alpha}_i = \frac{\alpha_0+2}{2}\widehat\lambda_i$.

To bound the estimation error for the linear classifier $\vct\eta$, we need to further bound $\varepsilon_{y,w}$.
We assume $\varepsilon_{y,w}\leq\varepsilon$.
By expanding $\varepsilon_{y,w}$ according to Definition \ref{def_epsilon} in a similar manner
we obtain the $(\|\vct\eta\|+\Phi^{-1}(\delta/60\sigma))^2$ term in the requirment of $n_2$.
The bound on $|\eta_i-\widehat\eta_{\pi(i)}|$ follows immediately by Lemma \ref{lem_eta}.

Finally, we bound $\|\vct\mu_i-\widehat{\vct\mu}_{\pi(i)}\|$ using Lemma \ref{lem_mu}.
We need to assume that $\frac{6\alpha_{\max}\sigma_1(\widetilde O)E_P}{\sigma_k(\widetilde O)^2} \leq \varepsilon$,
which gives the $\alpha_{\max}^2\sigma_1(\widetilde O)^2$ term. %in Eq. (\ref{eq_n2}).
The $\|\vct\mu_i-\widehat{\vct\mu}_{\pi(i)}\|$ bound then follows by Lemma \ref{lem_mu} and Lemma \ref{lem_tensorpower}.

\end{proof}

We make some remarks for the main theorem. In Remark~\ref{rem_connection}, we establish links between indirect quantities appeared in Theorem~\ref{thm_main} (e.g., $\sigma_k(\widetilde O)$) and the functions of original model parameters (e.g., $\sigma_k(O)$).
These connections are straightforward following their definitions.

\begin{rem}
The indirect quantities $\sigma_1(\widetilde O)$ and $\sigma_k(\widetilde O)$ can be related to $\sigma_1(O)$, $\sigma_k(O)$ and $\vct\alpha$ in the following way:
{\small \begin{equation*}
\sqrt{\frac{\alpha_{\min}}{\alpha_0(\alpha_0+1)}}\sigma_k(O) \leq \sigma_k(\widetilde O)\leq \sqrt{\frac{\alpha_{\max}}{\alpha_0(\alpha_0+1)}}\sigma_k(O);~~~~
\end{equation*}
\begin{equation*}
\sigma_1(\widetilde O) \leq \sqrt{\frac{\alpha_{\max}}{\alpha_0(\alpha_0+1)}}\sigma_1(O) \leq \frac{1}{\sqrt{\alpha_0+1}}.
\end{equation*}}
\label{rem_connection}
\end{rem}

We now take a close look at the sample complexity bound in Theorem~\ref{thm_main}.
It is evident that $n_2$ can be neglected when the number of topics $k$ gets large,
because in practice the norm of the linear regression model $\vct\eta$ is usually assumed to be small in order to avoid overfitting.
Moreover, as mentioned before, the prior parameter $\vct\alpha$ is often assumed to be homogeneous with $\alpha_i = 1/k$ \cite{lsa}.
With these observations, the sample complexity bound in Theorem~\ref{thm_main}
can be greatly simplified. %, as shown in Remark~\ref{rem_simpbound}.
\begin{rem}
Assume $\|\vct\eta\|$ and $\sigma$ are small and $\vct\alpha = (1/k, \cdots, 1/k)$.
As the number of topics $k$ gets large, the sample complexity bound in Theorem~\ref{thm_main} can be simplified as
\begin{equation}
N = \Omega\left( \frac{\log(1/\delta)}{\sigma_k(\widetilde O)^{10}}\cdot\max(\varepsilon^{-2}, k^3)\right).
\end{equation}\label{rem_simpbound}
\end{rem}\vspace{-.5cm}
The sample complexity bound in Remark~\ref{rem_simpbound} may look formidable
as it depends on $\sigma_k(\widetilde O)^{10}$.
However, such dependency is somewhat necessary because we are using third-order tensors to recover the underlying model parameters.
Furthermore, the dependence on $\sigma_k(\widetilde O)^{10}$ is introduced by the robust tensor power method to recover LDA parameters,
and the reconstruction accuracy of $\vct\eta$ only depends on $\sigma_k(\widetilde O)^4$ and $(\|\vct\eta\|+\Phi^{-1}(\delta/60\sigma))^2$.
As a consequence, if we can combine our power update method for $\vct \eta$ with LDA inference algorithms that have milder dependence on the singular value $\sigma_k(\widetilde O)$,
we might be able to get an algorithm with a better sample complexity.






%In summary, by applying the above trick, the number of operations needed to compute the whitened empirical moment
%$\widehat{\mathbb E}[\vct x_1\otimes\vct x_2\otimes\vct x_3](\widehat W,\widehat W,\widehat W)$
%can be reduced from $O(NV^3)$ to $O(N(Vk^2+k^3))$.

\iffalse
\section{Discussions}

\subsection{Appendix C.1. Extension to other topic recovery algorithms}

One important advantage of our proposed inference algorithm is its flexibility---the algorithm can be combined with many other LDA inference algorithms to infer supervised LDA model parameters.
More specifically, given access to any algorithm that recovers the topic distribution matrix $O$
and the prior parameter $\vct\alpha$ from i.i.d. sampled documents,
an inference algorithm for a supervised LDA model can be immediately obtained,
as shown in Algorithm \ref{alg2}.

\begin{algorithm}
\caption{sLDA parameter recovery based on an existing LDA inference algorithm $\mathcal A$. Input parameter: $\alpha_0$.}
\centering
\begin{algorithmic}[1]
%\Function{Recovery}{$\alpha_0$, $T$, $\Delta'$}
	\State Compute empirical moments and obtain $\widehat M_2, \widehat M_y$. Set $\widehat{\vct\eta} = 0$.
	\State Find $\widehat W\in\mathbb R^{n\times k}$ such that $\widehat M_2(\widehat W, \widehat W) = I_k$.
%	\State Find singular values and singular vectors $(\widehat\sigma_i^y, \widehat{\vct v}_i^y)$ of $\widehat M_y(\widehat W, \widehat W)$.
	\State Run algorithm $\mathcal A$ with observed documents and parameter $\alpha_0$. Obtain the estimated
topic distribution matrix $\widehat O=(\widehat{\vct\mu}_1,\cdots,\widehat{\vct\mu}_k)$ and prior parameter $\widehat{\vct\alpha}$.
	\State Compute $\widehat{\vct v}_i = \sqrt{\frac{\widehat{\alpha}_i}{\alpha_0(\alpha_0+1)}}\widehat W^\top\widehat{\vct\mu}_i$ for each topic $i$.
	\State Recover linear classifier: $\widehat\eta_i \gets \frac{\alpha_0+2}{2}\widehat{\vct v}_i^\top\widehat M_y(\widehat W,\widehat W)\widehat{\vct v}_i$.
	\State \textbf{Output:} $\widehat{\vct\eta}$, $\vct\alpha$ and $\{\widehat{\vct\mu}_i\}_{i=1}^k$.
%\EndFunction
\end{algorithmic}
\label{alg2}
\end{algorithm}

The sample complexity of Algorithm \ref{alg2} depends on the sample complexity of the LDA inference algorithm $\mathcal A$.
Although the LDA inference algorithm $\mathcal A$ is free to make any assumptions on the topic distribution matrix $O$,
we comment that the linear independence of topic distribution vectors $\vct\mu$ is still required,
because the power update trick (step 5 in Algorithm 1) is valid only $W\vct\mu_i$ are orthogonal vectors.
%\junx{Which algorithm 1, the main text or this one?}{\color{blue} fixed. all Algorithm 1 refers to this algorithm.}

\subsection*{Appendix C.2. Going beyond SVD}

The proposed methods are based on spectral decomposition of observable moments
and are provably correct.
However, a major drawback of these methods is their assumption that the topic distributions $\vct\mu$ are linearly independent.
Although standard LDA models assume this topic independence \cite{lda},
in practice there is strong evidence that different topics might be related \cite{correlatelda}.
Therefore, it is important to consider possible extensions.

Recently, there has been much work on provable LDA inference algorithms that do not require the topic independence assumption \cite{practicalalgo,beyondsvd}.
Instead of making the independence assumption, these methods assume a $p$-separability condition on the topic distribution matrix,
that is, there exists an \emph{anchor word} for each topic such that the anchor word only appears in this specific topic,
and its probability (given that topic) is at least $p$.

Here we briefly describe an idea that might lead to an sLDA inference algorithm without assuming topic independence.
First, let $O\in\mathbb R^{V\times k}$ be the topic distribution matrix defined previously and $H = (\vct h_1,\cdots,\vct h_N)\in\mathbb R^{k\times N}$
be the matrix of topic mixing vectors for each document.
Suppose $Q = \mathbb E[\vct x_1\vct x_2^\top]$ is the word co-occurrence frequency matrix
and $Q_y = \mathbb E[y\vct x_1]$ is the co-occurrence frequency matrix between word and regression variable observations.
It is clear that both $Q$ and $Q_y$ can be estimated from the training data, and we have
\begin{equation}
Q = ORO^\top, Q_y = OR\vct\eta,
\end{equation}
where $R \triangleq \mathbb E[HH^\top]$.

Assuming the $p$-separability condition holds and using methods developed in \cite{beyondsvd,practicalalgo},
we can consistently recover the $O$ and $R$.
Now note that $Q_y = (OR)\cdot \vct\eta$.
As a result, knowing both $OR$ and $Q_y$ we reduce the $\vct\eta$ inference problem to solving a linear equation systems.
Future research could be done on (1) determining when the matrix $OR$ has full rank $r$ so that the linear equations can be solved, and
(2) investigating the sample complexity problem for such an inference algorithm.

\subsection*{Appendix C.3. From regression to classification}

A natural extension to our result is to consider supervised LDA models for classification purposes.
The simplest model is a logistic regression classification model, where we assume the response variable $y_d$
for each document $d$ is in $\{+1,-1\}$, and
$$\Pr[y_d = 1|\vct h_d] = \frac{\exp(\vct\eta^\top\vct h_d)}{1+\exp(\vct\eta^\top\vct h_d)},$$
where $\vct\eta$ is a linear classifier.

Though appears simple, such an extension incurs many fundamental problems.
A major obstacle is the fact that the conditional expectation $\mathbb E[y|\vct h]$ is no longer linear
in the topic mixing vector $\vct h$.
As a result, we cannot even evaluate $\mathbb E[y]$ (or higher order tensors like $\mathbb E[y\vct x_1\otimes\vct x_2]$)
in closed forms.
Further more, even if we have accurate estimation to the above moments,
it is rather difficult to infer $\vct\eta$ back due to its non-linearality.
To our knowledge, the classification problem remains unsolved in terms of spectral decomposition methods,
and there is doubt whether a provably correct algorithm exists in such scenarios.
\fi



==> untitled folder/supplementary2.tex <==

\section{Proof of Theorem 2}
In this section we give the proof of Theorem 2, following the similar line of the proof of Theorem
1. We bound the estimation errors and the errors introduced by the tensor decomposition step
respectively.%\jun{please learn from Appendix A on how to using commas after equations. Basically, equations are part of a sentence, so commas are needed.}

\subsection{Definitions}
We first recall the definition of joint canconical topic distribution.
\begin{deff}
	(Joint Canconical topic distribution) Define the canconical version of joint topic distribution vector
	$\bm{v}_i,\widetilde{\bm{v}}_i$ as follows:
	$$
	\widetilde{\bm{v}}_i = \sqrt{\dfrac{\alpha_i}{\alpha_0(\alpha_0 +1)}}\bm{v}_i,
	$$
	where $\bm{v}_i = [ \bm{\mu}_i' , \eta_i]'$ is the topic dictribution vector extended by its regression parameter.

	We also define $O^*, \widetilde{O^*} \in \mathbb{R}^{(V+1) \times k}$ by $ O^* = [ \bm{v}_1, ... ,\bm{v}_k] $
	and $ \widetilde{O^*} = [ \widetilde{\bm{v}}_1 , ..., \widetilde{\bm{v}}_k]$.
		
\end{deff}
	

\subsection{Estimation Errors}
The tail inequatlities in last section \ref{lem_chernoff},\ref{cor_chernoff} gives the following estimation:
\begin{lem}
	\label{l1}
	Suppose we obtain $N$ i.i.d. samples. Let $\mathbb{E}[\cdot]$ denote the mean of the true underlying distribution and $\hat{\mathbb{E}}[\cdot]$ denote
	the empirical mean. Define
	\begin{equation}
	\begin{aligned}
		& R_1(\delta) = \|\bm{\eta}\| - \sigma\Phi^{-1}(\delta),\\
		& R_2(\delta) = 2\|\bm{\eta}\|^2 + 2\sigma^2[\Phi^{-1}(\delta)]^2, \\
		& R_3(\delta) = 4\|\bm{\eta}\|^3 - 4\sigma^3[\Phi^{-1}(\delta)]^3, \\
		%& R_4(\delta) = R_1(\delta) + R_2(\delta) + R_3(\delta)
	\end{aligned}
	\end{equation}
	where $\Phi^{-1}(\cdot)$ is the inverse function of the CDF of a
	standard Gaussian distribution. Then:
	\begin{equation}
	\begin{aligned}
		&	\Pr \left [ \| \mathbb{E}[ \mathbf{x_1} \otimes \mathbf{x_2} \otimes \mathbf{x_3}]  - \hat{\mathbb{E}}[\mathbf{x_1} \otimes
\mathbf{x_2} \otimes \mathbf{x_3} ] \|_F   < \dfrac{2 + \sqrt{2\log(1/\delta)} }{ \sqrt{N}}  \right ]  \geq 1 - \delta; \\
												   &		\Pr \left [ \| \mathbb{E}[ y^i ]  - \hat{\mathbb{E}}[ y^i ] \|_F < R_i(\delta/4 N )\cdot
			 \dfrac{2 + \sqrt{2\log(2/\delta)} }{ \sqrt{N} } \right ]  \geq 1 - \delta  \ \ \ \ i = 1, 2, 3;\\
			 & 		\Pr \left [ \| \mathbb{E}[  y^i \mathbf{x_1} ]  - \hat{\mathbb{E}}[ y^i \mathbf{x_1}  ] \|_F
				 < R_i(\delta / 4 N) \cdot \dfrac{2 + \sqrt{2\log(2/\delta)} }{ \sqrt{N}} \right ]  \geq 1 - \delta  \ \ \ \ i = 1,2;\\
				 & 		\Pr \left [ \| \mathbb{E}[  y^i \mathbf{x_1} \otimes \mathbf{x_2} ]  - \hat{\mathbb{E}}[ y^i \mathbf{x_1} \otimes \mathbf{x_2} ] \|_F
				 < R_i(\delta / 4 N) \cdot \dfrac{2 + \sqrt{2\log(2/\delta)} }{ \sqrt{N}} \right ]  \geq 1 - \delta  \ \ \ \ i = 1 , 2.\\
	\end{aligned}
	\end{equation}
\end{lem}
\begin{proof}
	This lemma is a direct application of lemma \ref{lem_chernoff} and corollary \ref{cor_chernoff}.
\end{proof}

\begin{cor}
\label{c1}
	With probability $1 -\delta$, the following holds:
	\begin{equation}
	\begin{aligned}
		& Pr  \left [ \| \mathbb{E}[ \mathbf{z_1}] - \hat{\mathbb{E}}[ \mathbf{z_1}] \| < C_1(\delta / 8 N)
			\dfrac{2 + \sqrt{2\log(4/\delta)} }{ \sqrt{N}}   \right ] \geq 1 - \delta,   \\
			& Pr  \left [ \| \mathbb{E}[ \mathbf{z_1} \otimes \mathbf{z_2}] - \hat{\mathbb{E}}[ \mathbf{z_1} \otimes \mathbf{z_2}] \|   < C_2(\delta / 12 N)
		\dfrac{2 + \sqrt{2\log(6/\delta)} }{ \sqrt{N}}   \right ]   \geq 1 - \delta,   \\
		&	Pr  \left [ \| \mathbb{E}[ \mathbf{z_1} \otimes \mathbf{z_2} \otimes \mathbf{z_3}]  - \hat{\mathbb{E}}[\mathbf{z_1} \otimes
	\mathbf{z_2} \otimes \mathbf{z_3} ] \|_F   < C_3(\delta/16N) \dfrac{2 + \sqrt{2\log(8/\delta)} }{ \sqrt{N}}   \right ]  \geq 1 - \delta, \\
	\end{aligned}
	\end{equation}
	where
	\begin{equation}
	\begin{aligned}
		& C_1(\delta) = R_1(\delta) + 1, \\
		& C_2(\delta) = R_1(\delta) + R_2(\delta) + 1, \\
		& C_3(\delta) = R_1(\delta) + R_2(\delta) + R_3(\delta) + 1. \\
	\end{aligned}
	\end{equation}
\end{cor}
\begin{proof}
	Use lemma \ref{l1} as well as the fact that $\sqrt{a + b} \leq \sqrt{a} + \sqrt{b}, \forall a,b \geq 0$ and $ Pr( X \leq t_1 , Y \leq t_2) \leq Pr( X + Y \leq t_1 + t_2)$.
\end{proof}

\begin{lem}
\label{l3}
	(concentration of moment norms) Using notations in lemma \ref{l1} and suppose
	$C_3(\delta/144N)\dfrac{2 +\sqrt{2\log(72/\sigma)}}{\sqrt{N}} \leq 1 $
	we have:
	\begin{equation}
	\begin{aligned}
		& E_P = \|N_2 - \hat{N}_2\| \leq 3C_2(\delta/36N)) \cdot 	\dfrac{2 + \sqrt{2 \log(18/\sigma)}}{\sqrt{N}},\\
		& E_T = \|N_3 - \hat{N}_3\| \leq 10C_3(\delta/144N)) \cdot  \dfrac{2 + \sqrt{2 \log(72/\sigma)}}{\sqrt{N}}.\\
	\end{aligned}
	\end{equation}
\end{lem}
\begin{proof}
	This lemma can be proved by expanding the terms by definition and use lemma \ref{l1} , corollary \ref{c1} as well as union bound.
	Also note that $\| \cdot\| \leq \|\cdot \|_F$.
\end{proof}

\begin{lem}
	(estimation error of whitened moments)
	Define
	\begin{equation}
	\begin{aligned}
		& \epsilon_{p,w} = \| N_2(W,W) - \hat{N}_2(\hat{W},\hat{W})\|, \\
		& \epsilon_{t,w} = \| N_3(W,W,W) - \hat{N}_3(\hat{W},\hat{W},\hat{W})\|. \\
	\end{aligned}
	\end{equation}
	Then we have:
	\begin{equation}
	\begin{aligned}
		& \epsilon_{p,w} \leq  \dfrac{16E_p}{\sigma_k(\widetilde{O^*})^2}, \\
		& \epsilon_{t,w} \leq  \dfrac{54E_P}{(\alpha_0+1)(\alpha_0+2)\sigma_k(\widetilde{O^*})^5} +
		\dfrac{8E_T}{\sigma_k(\widetilde{O^*})^3}.
	\end{aligned}
	\end{equation}
\end{lem}

\subsection{SVD accuracy}

We rewrite a part of Lemma ~\ref{lem_whiten} which we will use in the following.

\begin{lem}
\label{l5}
	Let $W,\hat{W} \in R^{(V+1)\times k}$ be the whitening matrices such that
		$N_2(W,W) = \hat{W}_2(\hat{W},\hat{W}) = I_k$. Further more, we suppose
		$ E_P \leq \sigma_k(N_2)/2$. Then we have:
		\begin{equation}
		\begin{aligned}
			& \|W - \hat{W}\| \leq \dfrac{4E_P}{\sigma_k(\widetilde{O^*})^3},\\
			& \|W^+\| \leq 3\sigma_1(\widetilde{O^*}), \\
			& \|\widetilde{W}^+\| \leq 2\sigma_1(\widetilde{O^*}), \\
			& \|W^+ - \hat{W}^+\| \leq \dfrac{6\sigma_1(\widetilde{O^*})E_P}{\sigma_k(\widetilde{O^*})^2}.\\
		\end{aligned}
		\end{equation}
\end{lem}


Using the above lemma, we now can estimate the error introduced by SVD.

\begin{lem}($\bm{v}_i$ estimation error)
\label{l6}
	Define $\hat{\bm{v}}_i = \frac{\alpha_0 + 2}
	{2}\hat{\lambda}_i(\hat{W}^+)^{\top}\hat{\bm{\omega}}_i$ where
	 $(\hat{\lambda}_i,\hat{\omega}_i)$ are some estimations of svd pairs
	 $(\lambda_i, \omega_i)$ of $ N_3(W,W,W)$. We then have:
	\begin{equation}
	 \begin{aligned}
		 \|\hat{\bm{v}}_i - \bm{v}_i\| \leq& \dfrac{(\alpha_0 + 1)6\sigma_1(\widetilde{O^*})E_P}{\sigma_k(\widetilde{O^*})^2}
		 + \dfrac{(\alpha_0 +2)\sigma_1(\widetilde{O^*})|\hat{\lambda}_i - \lambda_i|}{2}
	 +3(\alpha_0 +1)\sigma_1(\widetilde{O^*})\|\hat{\bm{\omega}}_i - \bm{\omega}_i\|.
	\end{aligned}
	 \end{equation}
\end{lem}

\begin{proof}
	Note that $\bm{v}_i = \frac{}{}\lambda_i(W^+)^{\top}\bm{\omega}_i$. Thus we have:
	\begin{equation}
	\begin{aligned}
		\frac{2}{\alpha_0 + 2 } \|\hat{\bm{v}}_i - \bm{v}_i\|
		= &\|\hat{\lambda}_i(\hat{W}^+)^{\top}\hat{\bm{\omega}_i}
		- \lambda_i(W^+)^{\top}\bm{\omega}_i \| \\
		=& \|\hat{\lambda}_i(\hat{W}^+)^{\top}\hat{\bm{\omega}_i}
		- \lambda_i(W^+)^{\top}\hat{\bm{\omega}}_i
		+ \lambda_i(W^+)^{\top}\hat{\bm{\omega}}_i
		- \lambda_i(W^+)^{\top}\bm{\omega}_i \| \\
		\leq& \|\hat{\lambda}_i(\hat{W}^+)^{\top} - \lambda_i(W^+)^{\top}\|
			\|\hat{\bm{\omega}}_i\|
			+ \|\lambda_i(W^+)^{\top}\|\|\hat{\bm{\omega}}_i - \bm{\omega}_i\|\\
			\leq& |\lambda_i|\|\hat{W}^+ - W^+\|
			\|\hat{\bm{\omega}}_i\| +
			|\hat{\lambda}_i - \lambda_i|\|\hat{W}^+\|
			\|\hat{\bm{\omega}}_i\|
			+ |\lambda_i|\|W^+\|\|\hat{\bm{\omega}}_i - \bm{\omega}_i\|\\
			\leq& \dfrac{2(\alpha_0 +1)}{\alpha_0 + 2}\dfrac{6E_P\sigma_1(\widetilde{O^*})}{\sigma_k(\widetilde{O^*})^2}
			+ 3\sigma_1(\widetilde{O^*})|\hat{\lambda}_i - \lambda_i| +
			\dfrac{2(\alpha_0 + 1)}{\alpha_0 + 2}\cdot
			3\sigma_1(\widetilde{O^*})\cdot \|\hat{\bm{\omega}}_i - \bm{\omega}_i \|.
	\end{aligned}
	\end{equation}
\end{proof}

\iffalse
We now cite an lemma from \cite{a:tensor} that provides a bound for the estimation error of $\bm{\omega}_i$
and $\lambda_i$.

\begin{lem}
\label{l7}
	Let $\lambda_{max} =
		\frac{2}{\alpha_0 + 2}\sqrt{\dfrac{\alpha_0(\alpha_0 + 1)}{\alpha_{min}}}$ and
	 $\lambda_{min} =
		\frac{2}{\alpha_0 + 2}\sqrt{\dfrac{\alpha_0(\alpha_0 + 1)}{\alpha_{max}}}$, where
	$\alpha_{max} = \max \alpha_i ,\alpha_{min} = \min \alpha_i$. Then there exist universal
	constants $C_1,C_2 > 0$ such that the following hods: Fix $\delta' \in ( 0,1)$. Suppose
	$\epsilon_{t,w} \leq \epsilon$ and
	$$
	\epsilon_{t,w} \leq C_1 \cdot \dfrac{\lambda_{min}}{k}
	$$

Suppose $\{(\hat{\lambda}_i, \hat{\bm{v}}_i\}_{i=1}^{k}\}$ are eigenvalue and eigenvector pairs
returned by running Algorithm $1$ in \cite{a:tensor} with input $\hat{W}_3(\hat{W},\hat{W},\hat{W}) $ for
$L = poly(k)\log(1/\delta')$ and $N \geq C_2\cdot (\log(k) +
\log\log(\frac{\lambda_{max}}{\epsilon}) $ iterations. With probability at least $1 - \delta'$,
there exists a permutation $\pi':[k]\to[k]$ such that for all i:
$$
\|\hat{\bm{\omega}}_i - \bm{\omega}_i\| \leq 8\epsilon / \lambda_{min}, |\hat{\lambda}_i - \lambda_i | \leq 5 \epsilon.
$$
\end{lem}
\fi


\subsection{Completeing the proof}
We are now ready to complete the proof of Theorem ~\ref{thm_main2}. %\jun{inconsistent with the main text.}
\iffalse
\begin{theorem}
	(Sample complexity bound)
	Let $ \sigma_1(\widetilde{O^*})$ and $\sigma_k(\widetilde{O^*})$ be the largest and smallest singular
	values of the joint canonical topic dictribution matrix $\widetilde{O^*}$.

	For any error-tolerance parameter $\epsilon > 0$, if Algorithm $1$ runs  at least
	$T = \Omega(\log(k)) + \log\log(\dfrac{\lambda_{max}}{\epsilon})$ iterations on $N$ i.i.d. sampled documents with $N$
	satisying:
	\begin{equation}
	\begin{aligned}
		& N \geq K_1 \cdot  \dfrac{\alpha_0^2(\alpha_0+1)^2C_2^2(\delta/36N)\cdot(2 + \sqrt{2\log(18/\delta)})^2 }{\alpha_{min}^2}	 \\
		& N \geq  K_2 \cdot C_3^2(\delta/144N)(2 + \sqrt{2 \log(72/\sigma)})^2   \\
		&N \geq K_3 \cdot \dfrac{C_3^2(\delta/36N)(2+\sqrt{2\log(18/\sigma)})^2}
			{\sigma_k(\widetilde{O^*})^{10}}\cdot\max(\dfrac{1}{\epsilon^2}, \dfrac{k^2}{\lambda_{min}^2})\\
	\end{aligned}
	\end{equation}
	then with probability at least $1 - \delta$, there exist a permutation $\pi: [k] \to [k]$
	such that the following holds for every $i \in [k]$:
	\begin{equation}
	\begin{aligned}
	& |\alpha_i - \hat{\alpha}_{\pi(i)} |
			\leq \dfrac{4\alpha_0(\alpha_0 + 1) }{(\alpha_0 + 2)^2\lambda_{min}^2(\lambda_{min} - 5 \epsilon)^2} \cdot 5\epsilon \\
			& \|\bm{v}_i - \hat{\bm{v}}_{\pi(i)}  \|	\leq \left ( \sigma_1(\widetilde{O^*})(\alpha_0  + 2)(\frac{7}{2} +
	\frac{8}{\lambda_{min}})\right )\cdot \epsilon \\
	\end{aligned}
	\end{equation}
\end{theorem}
\fi

\begin{proof}{(Proof of Theorem~\ref{thm_main2})}
	We check out the conditions that must be satisfied for $\epsilon$ accuracy.
	First $E_P \leq \sigma_k(N_2)/2$ is required in lemma \ref{l5}. Noting that $\sigma_k(N_2) = \dfrac{\alpha_{min}}{\alpha_0(\alpha_0 + 1)} $, we have:
	$$
		N \geq O\left (  \dfrac{\alpha_0^2(\alpha_0+1)^2C_2^2(\delta/36N)\cdot(2 + \sqrt{2\log(18/\delta)})^2 }{\alpha_{min}^2}\right ).
	$$
	In lemma \ref{l3}, we need that $C_3(\delta/144N)\dfrac{2\log(72/\sigma)}{\sqrt{N}} \leq 1$, which means:
	$$
		N \geq O \left ( C_3^2(\delta/144N)(2 + \sqrt{2 \log(72/\sigma)})^2 \right ).
	$$
	For lemma \ref{lem_tensorpower} to hold, we need the assumption that $\epsilon_{t,w} \leq C_1 \cdot \frac{\lambda_{min}}{k}$, which implies:
	$$
		N \geq 	O \left ( \dfrac{C_3^2(\delta/36N)(2+\sqrt{2\log(18/\sigma)})^2}{\sigma_k(\widetilde{O^*})^{10}}\cdot\max(\dfrac{1}{\epsilon^2},
		\dfrac{k^2}{\lambda_{min}^2}) \right ).
	$$

	From the recovery rule $\hat{\alpha_i} = \dfrac{4\alpha_0(\alpha_0 + 1)}{(\alpha_0 + 2)^2 \hat{\lambda_i}^2}$, we have:
	\begin{equation}
	\begin{aligned}
		 |\hat{\alpha}_i - \alpha_i |
		  \leq \dfrac{4\alpha_0(\alpha_0 + 1) }{(\alpha_0 + 2)^2}
		\left |\dfrac{1}{\hat{\lambda}_i^2} - \dfrac{1}{\lambda_i^2} \right |
		\leq \dfrac{4\alpha_0(\alpha_0 + 1) }{(\alpha_0 + 2)^2\lambda_{min}^2(\lambda_{min} - 5 \epsilon)^2} \cdot 5\epsilon. \\
	\end{aligned}
	\end{equation}
	Finally, we bound $\|\hat{\bm{v}}_i - \bm{v}_i\|$, which is a direct consequence of lemma \ref{l6} and lemma \ref{lem_tensorpower}.
	We additional assume the following condition holds: $\dfrac{6E_P}{\sigma_k(\widetilde{O^*})^2} \leq \epsilon $. In fact, this condition is already satisfied
	if the above requirements for $N$ hold.
	Under this condition, we have:
	$$
	\|\hat{\bm{v}}_i - \bm{v}_i \|	\leq \left ( \sigma_1(\widetilde{O^*})(\alpha_0  + 2)(\frac{7}{2} +
	\frac{8}{\lambda_{min}})\right )\cdot \epsilon.\\
	$$
\end{proof}




==> untitled folder/supplementary3.tex <==
\section{Moments of Observable Variables}

\subsection{Proof to Proposition 1}

The equations on $M_2$ and $M_3$ have already been proved in \cite{speclda} and \cite{a:tensordecomp}.
Here we only give the proof to the equation on $M_y$.
In fact, all the three equations can be proved in a similar manner.

In sLDA the topic mixing vector $\vct h$ follows a Dirichlet prior distribution with parameter $\vct\alpha$.
Therefore, we have
\begin{equation}
\begin{aligned}
	&\mathbb E[h_i] = \frac{\alpha_i}{\alpha_0},\\
 &\mathbb E[h_ih_j] = \left\{\begin{array}{ll} \frac{\alpha_i^2}{\alpha_0(\alpha_0+1)}, &\text{if }i=j,\\
\frac{\alpha_i\alpha_j}{\alpha_0^2}, &\text{if }i\neq j\end{array}\right.,\\
									 &\mathbb E[h_ih_jh_k] = \left\{\begin{array}{ll} \frac{\alpha_i^3}{\alpha_0(\alpha_0+1)(\alpha_0+2)}, & \text{if }i=j=k,\\
\frac{\alpha_i^2\alpha_k}{\alpha_0^2(\alpha_0+1)}, & \text{if }i=j\neq k,\\
\frac{\alpha_i\alpha_j\alpha_k}{\alpha_0^3}, &\text{if }i\neq j, j\neq k, i\neq k\end{array}\right. .
\end{aligned}
\end{equation}

Next, note that
\begin{equation}
\begin{aligned}
	&\mathbb E[y|\vct h] = \vct\eta^\top\vct h,\\
 &\mathbb E[\vct x_1|\vct h] = \sum_{i=1}^k{h_i\vct\mu_i},\\
 &\mathbb E[\vct x_1\otimes\vct x_2|\vct h] = \sum_{i, j=1}^k{h_ih_j\vct\mu_i\otimes\vct\mu_j},\\
 &\mathbb E[y\vct x_1\otimes\vct x_2|\vct h] = \sum_{i, j, k=1}^k{h_ih_jh_k\cdot \eta_k\vct\mu_j\otimes\vct\mu_k}.
\end{aligned}
\end{equation}

Proposition 1 can then be proved easily by taking expectation over the topic mixing vector $\vct h$.

\subsection{Details of the speeding-up trick}

In this section we provide details of the trick mentioned in the main paper to speed up empirical moments computations.
First, note that the computation of $\widehat M_1$, $\widehat M_2$ and $\widehat M_y$ only requires $O(NM^2)$ time and $O(V^2)$ space.
They do not need to be accelerated in most practical applications.
This time and space complexity also applies to all terms in $\widehat M_3$ except the $\widehat{\mathbb E}[\vct x_1\otimes\vct x_2\otimes\vct x_3]$ term,
which requires $O(NM^3)$ time and $O(V^3)$ space if using naive implementations.
Therefore, this section is devoted to speed-up the computation of $\widehat{\mathbb E}[\vct x_1\otimes\vct x_2\otimes\vct x_3]$.
More precisely, as mentioned in the main paper,
what we want to compute is the whitened empirical moment $\widehat{\mathbb E}[\vct x_1\otimes\vct x_2\otimes\vct x_3](\widehat W,\widehat W,\widehat W) \in
\mathbb R^{k\times k\times k}$.

Fix a document $D$ with $m$ words.
Let $T \triangleq \widehat{\mathbb E}[\vct x_1\otimes\vct x_2\otimes\vct x_3|D]$ be the empirical tensor demanded.
By definition, we have

\begin{equation}
T_{i,j,k} = \frac{1}{m(m-1)(m-2)}\left\{\begin{array}{ll}
n_i(n_j-1)(n_k-2),& i=j=k;\\
n_i(n_i-1)n_k,& i=j,j\neq k;\\
n_in_j(n_j-1),& j=k,i\neq j;\\
n_in_j(n_i-1),& i=k,i\neq j;\\
n_in_jn_k,& \text{otherwise};\end{array}\right.
\label{eq_T}
\end{equation}
where $n_i$ is the number of occurrences of the $i$-th word in document $D$.
If $T_{i,j,k} = \frac{n_in_jn_k}{m(m-1)(m-2)}$ for all indices $i,j$ and $k$,
then we only need to compute
$$T(W,W,W) = \frac{1}{m(m-1)(m-2)}\cdot (W\vct n)^{\otimes 3},$$
where $\vct n \triangleq (n_1,n_2,\cdots,n_V)$.
This takes $O(Mk + k^3)$ computational time because $\vct n$ contains at most $M$ non-zero entries,
and the total time complexity is reduced from $O(NM^3)$ to $O(N(Mk+k^3))$.

We now consider the remaining values, where at least two indices are identical.
We first consider those values with two indices the same, for example, $i=j$.
For these indices, we need to subtract an $n_in_k$ term, as shown in Eq. (\ref{eq_T}).
That is, we need to compute the whitened tensor $\Delta(W,W,W)$, where $\Delta\in\mathbb R^{V\times V\times V}$ and
\begin{equation}
\Delta_{i,j,k} = \frac{1}{m(m-1)(m-2)}\cdot \left\{\begin{array}{ll}
n_in_k,& i=j;\\
0,& \text{otherwise}.\end{array}\right.
\end{equation}

Note that $\Delta$ can be written as $\frac{1}{m(m-1)(m-2)}\cdot A\otimes\vct n$,
where $A = \text{diag}(n_1,n_2,\cdots,n_V)$ is a $V\times V$ matrix and $\vct n = (n_1,n_2,\cdots,n_V)$ is defined previously.
As a result, $\Delta(W,W,W) = \frac{1}{m(m-1)(m-2)}\cdot (W^\top AW)\otimes \vct n$.
So the computational complexity of $\Delta(W,W,W)$ depends on how we compute $W^\top AW$.
Since $A$ is a diagonal matrix with at most $M$ non-zero entries, $W^\top AW$ can be computed in $O(Mk^2)$ operations.
Therefore, the time complexity of computing $\Delta(W,W,W)$ is $O(Mk^2)$ per document.

Finally we handle those values with three indices the same, that is, $i=j=k$.
As indicated by Eq. (\ref{eq_T}), we need to add a $\frac{2n_i}{m(m-1)(m-2)}$ term for compensation.
This can be done efficiently by first computing $\widehat{\mathbb E}(\frac{2n_i}{m(m-1)(m-2)})$
for all the documents (requiring $O(NV)$ time),
and then add them up, which takes $O(Vk^3)$ operations.








%In summary, by applying the above trick, the number of operations needed to compute the whitened empirical moment
%$\widehat{\mathbb E}[\vct x_1\otimes\vct x_2\otimes\vct x_3](\widehat W,\widehat W,\widehat W)$
%can be reduced from $O(NV^3)$ to $O(N(Vk^2+k^3))$.

\iffalse
\section{Discussions}

\subsection{Appendix C.1. Extension to other topic recovery algorithms}

One important advantage of our proposed inference algorithm is its flexibility---the algorithm can be combined with many other LDA inference algorithms to infer supervised LDA model parameters.
More specifically, given access to any algorithm that recovers the topic distribution matrix $O$
and the prior parameter $\vct\alpha$ from i.i.d. sampled documents,
an inference algorithm for a supervised LDA model can be immediately obtained,
as shown in Algorithm \ref{alg2}.

\begin{algorithm}
\caption{sLDA parameter recovery based on an existing LDA inference algorithm $\mathcal A$. Input parameter: $\alpha_0$.}
\centering
\begin{algorithmic}[1]
%\Function{Recovery}{$\alpha_0$, $T$, $\Delta'$}
	\State Compute empirical moments and obtain $\widehat M_2, \widehat M_y$. Set $\widehat{\vct\eta} = 0$.
	\State Find $\widehat W\in\mathbb R^{n\times k}$ such that $\widehat M_2(\widehat W, \widehat W) = I_k$.
%	\State Find singular values and singular vectors $(\widehat\sigma_i^y, \widehat{\vct v}_i^y)$ of $\widehat M_y(\widehat W, \widehat W)$.
	\State Run algorithm $\mathcal A$ with observed documents and parameter $\alpha_0$. Obtain the estimated
topic distribution matrix $\widehat O=(\widehat{\vct\mu}_1,\cdots,\widehat{\vct\mu}_k)$ and prior parameter $\widehat{\vct\alpha}$.
	\State Compute $\widehat{\vct v}_i = \sqrt{\frac{\widehat{\alpha}_i}{\alpha_0(\alpha_0+1)}}\widehat W^\top\widehat{\vct\mu}_i$ for each topic $i$.
	\State Recover linear classifier: $\widehat\eta_i \gets \frac{\alpha_0+2}{2}\widehat{\vct v}_i^\top\widehat M_y(\widehat W,\widehat W)\widehat{\vct v}_i$.
	\State \textbf{Output:} $\widehat{\vct\eta}$, $\vct\alpha$ and $\{\widehat{\vct\mu}_i\}_{i=1}^k$.
%\EndFunction
\end{algorithmic}
\label{alg2}
\end{algorithm}

The sample complexity of Algorithm \ref{alg2} depends on the sample complexity of the LDA inference algorithm $\mathcal A$.
Although the LDA inference algorithm $\mathcal A$ is free to make any assumptions on the topic distribution matrix $O$,
we comment that the linear independence of topic distribution vectors $\vct\mu$ is still required,
because the power update trick (step 5 in Algorithm 1) is valid only $W\vct\mu_i$ are orthogonal vectors.
%\junx{Which algorithm 1, the main text or this one?}{\color{blue} fixed. all Algorithm 1 refers to this algorithm.}

\subsection*{Appendix C.2. Going beyond SVD}

The proposed methods are based on spectral decomposition of observable moments
and are provably correct.
However, a major drawback of these methods is their assumption that the topic distributions $\vct\mu$ are linearly independent.
Although standard LDA models assume this topic independence \cite{lda},
in practice there is strong evidence that different topics might be related \cite{correlatelda}.
Therefore, it is important to consider possible extensions.

Recently, there has been much work on provable LDA inference algorithms that do not require the topic independence assumption \cite{practicalalgo,beyondsvd}.
Instead of making the independence assumption, these methods assume a $p$-separability condition on the topic distribution matrix,
that is, there exists an \emph{anchor word} for each topic such that the anchor word only appears in this specific topic,
and its probability (given that topic) is at least $p$.

Here we briefly describe an idea that might lead to an sLDA inference algorithm without assuming topic independence.
First, let $O\in\mathbb R^{V\times k}$ be the topic distribution matrix defined previously and $H = (\vct h_1,\cdots,\vct h_N)\in\mathbb R^{k\times N}$
be the matrix of topic mixing vectors for each document.
Suppose $Q = \mathbb E[\vct x_1\vct x_2^\top]$ is the word co-occurrence frequency matrix
and $Q_y = \mathbb E[y\vct x_1]$ is the co-occurrence frequency matrix between word and regression variable observations.
It is clear that both $Q$ and $Q_y$ can be estimated from the training data, and we have
\begin{equation}
Q = ORO^\top, Q_y = OR\vct\eta,
\end{equation}
where $R \triangleq \mathbb E[HH^\top]$.

Assuming the $p$-separability condition holds and using methods developed in \cite{beyondsvd,practicalalgo},
we can consistently recover the $O$ and $R$.
Now note that $Q_y = (OR)\cdot \vct\eta$.
As a result, knowing both $OR$ and $Q_y$ we reduce the $\vct\eta$ inference problem to solving a linear equation systems.
Future research could be done on (1) determining when the matrix $OR$ has full rank $r$ so that the linear equations can be solved, and
(2) investigating the sample complexity problem for such an inference algorithm.

\subsection*{Appendix C.3. From regression to classification}

A natural extension to our result is to consider supervised LDA models for classification purposes.
The simplest model is a logistic regression classification model, where we assume the response variable $y_d$
for each document $d$ is in $\{+1,-1\}$, and
$$\Pr[y_d = 1|\vct h_d] = \frac{\exp(\vct\eta^\top\vct h_d)}{1+\exp(\vct\eta^\top\vct h_d)},$$
where $\vct\eta$ is a linear classifier.

Though appears simple, such an extension incurs many fundamental problems.
A major obstacle is the fact that the conditional expectation $\mathbb E[y|\vct h]$ is no longer linear
in the topic mixing vector $\vct h$.
As a result, we cannot even evaluate $\mathbb E[y]$ (or higher order tensors like $\mathbb E[y\vct x_1\otimes\vct x_2]$)
in closed forms.
Further more, even if we have accurate estimation to the above moments,
it is rather difficult to infer $\vct\eta$ back due to its non-linearality.
To our knowledge, the classification problem remains unsolved in terms of spectral decomposition methods,
and there is doubt whether a provably correct algorithm exists in such scenarios.
\fi


